Narrowing the Gap between Zero- and Few-shot Machine Translation by Matching Styles

Large language models trained primarily in a monolingual setting have demonstrated their ability to generalize to machine translation using zero- and few-shot examples with in-context learning. However, even though zero-shot translations are relatively good, there remains a discernible gap comparing their performance with the few-shot setting. In this paper, we investigate the factors contributing to this gap and find that this gap can largely be closed (for about 70%) by matching the writing styles of the target corpus. Additionally, we explore potential approaches to enhance zero-shot baselines without the need for parallel demonstration examples, providing valuable insights into how these methods contribute to improving translation metrics.

==> emnlp2023-latex/qual_example.tex <==

qualitative examples to plot teaser figure and comet score range:
{
    "src": "Nach Artikel 34 Absatz 1 bis kann jede regionale Organisation zur wirtschaftlichen Integration Vertragspartei des Abkommens werden.",
    "tgt": "Whereas, under Article 34 (1bis), the Convention is open to accession by regional economic integration organizations;",
    "bm": "Under Article 34 (1 bis), the Convention is open to accession by regional economic integration organizations.",
    "style": "According to Article 34, paragraph 1, any regional organization for economic integration can become a party to the agreement.",
    "zeroshot": "According to Article 34, paragraph 1 to, any regional organization for economic integration can become a party to the agreement.",
    "bm_bleu": 0.7118329294072574,
    "style_bleu": 6.627196503686016e-155,
    "zeroshot_bleu": 6.4781755519555515e-155,
    "bm_comet": 0.9107282161712646,
    "style_comet": 0.8352534174919128,
    "zeroshot_comet": 0.7935122847557068,
    "src_retrieve_de": "Nach Artikel 33 Absatz 2 bis kann jede regionale Organisation zur wirtschaftlichen Integration Vertragspartei des Abkommens werde
n.",
    "src_retrieve_en": "Whereas under Article 33 (2 bis), the Convention is open to accession by regional economic integration organizations;",
    "tgt_retrieve": "Failing such acceptance, the State or regional economic integration organization making the reservation shall not become a party to 
this Agreement.",
    "comet_diff": 0.0754747986793518
}
{
    "src": "(121) Es wird die Auffassung vertreten, dass durch die Einf\u00fchrung von Ma\u00dfnahmen ein lauterer Wettbewerb auf dem Markt wiederhergest
ellt werden wird.",
    "tgt": "(121) It is considered that the imposition of measures will restore fair competition on the market.",
    "bm": "(121) It is considered that the imposition of measures will restore fair competition to the market.",
    "style": "It is believed that the introduction of measures will restore fair competition to the market.",
    "zeroshot": "It is believed that by introducing measures, fair competition will be restored in the market.",
    "bm_bleu": 0.8492326635760689,
    "style_bleu": 0.37116618872423884,
    "zeroshot_bleu": 3.4165878840545416e-78,
    "bm_comet": 0.9493653178215027,
    "style_comet": 0.8978716731071472,
    "zeroshot_comet": 0.8838595151901245,
    "src_retrieve_de": "(197) Es wird die Auffassung vertreten, dass durch die Einf\u00fchrung von Ma\u00dfnahmen ein lauterer Wettbewerb auf dem Markt w
iederhergestellt werden wird.",
    "src_retrieve_en": "(197) It is considered that the imposition of measures will restore fair competition to the market.",
    "tgt_retrieve": "(197) It is considered that the imposition of measures will restore fair competition to the market.",
    "comet_diff": 0.05149364471435547
}
{
    "src": "Sie m\u00fcssen aus einem Betrieb, einem Zentrum oder einer Einrichtung stammen, die regelm\u00e4ssigen amtlichen Veterin\u00e4rkontrollen ge
m\u00e4\u00df Absatz 3 unterworfen sind.",
    "tgt": "they must come from holdings, centres or organizations which are subject to regular official veterinary checks in accordance with paragraph 3
;",
    "bm": "They must come from a holding, centre or establishment which is subject to regular official veterinary checks in accordance with paragraph 3."
,
    "style": "They must come from an establishment, center, or facility subject to regular official veterinary inspections in accordance with paragraph 3
.",
    "zeroshot": "They must come from an operation, a center, or a facility that is subject to regular official veterinary inspections in accordance with 
paragraph 3.",
    "bm_bleu": 0.5489938756679379,
    "style_bleu": 0.42662196623863147,
    "zeroshot_bleu": 0.3595597536132021,
    "bm_comet": 0.905632495880127,
    "style_comet": 0.8786637187004089,
    "zeroshot_comet": 0.8582592606544495,
    "src_retrieve_de": "Es empfiehlt sich, ein Verfahren zur Beilegung von Streitf\u00e4llen, die im Zusammenhang mit Sendungen aus einem Betrieb, einem 
Zentrum oder einer Einrichtung auftreten k\u00f6nnen, festzulegen.",
    "src_retrieve_en": "Whereas provision should be made for a procedure for resolving conflicts which could arise concerning consignments from a holding
, centre or organization;",
    "tgt_retrieve": "They must come from a holding placed under veterinary supervision.",
    "comet_diff": 0.026968777179718018
}
{
    "src": "(5) Der Kooperationsausschuss fasst seine Beschl\u00fcsse einstimmig.",
    "tgt": "5. The Cooperation Committee shall take decisions by common accord.",
    "bm": "5. The Cooperation Committee takes its decisions unanimously.",
    "style": "The Cooperation Committee adopts its decisions unanimously.",
    "zeroshot": "The cooperation committee passes its resolutions unanimously.",
    "bm_bleu": 0.2644967217413845,
    "style_bleu": 3.486509539245492e-78,
    "zeroshot_bleu": 3.297337141451012e-78,
    "bm_comet": 0.8586069941520691,
    "style_comet": 0.8511139154434204,
    "zeroshot_comet": 0.7365868091583252,
    "src_retrieve_de": "(5) Der Verwaltungsrat fasst seine Beschl\u00fcsse mit der einfachen Mehrheit der Vertreter der Mitgliedstaaten.",
    "src_retrieve_en": "5. The Administrative Board shall take its decisions by a simple majority of the representatives of the Member States.",
    "tgt_retrieve": "5. The committee shall, where necessary, submit motions for resolutions to Parliament on petitions which it has considered.",
    "comet_diff": 0.007493078708648682
}



# different comet quality for few-shot
"src": "(3) Die pers\u00f6nliche Haftung der Bediensteten gegen\u00fcber der Beobachtungsstelle bestimmt sich nach den f\u00fcr das Personal der Beobachtungsstelle geltenden Vorschriften.",
"tgt": "3. The personal liability of servants towards the Centre shall be governed by the provisions applying to the staff of the Centre.",
"bm": "3. The personal liability of servants towards the Observatory shall be governed by the provisions applying to the staff of the Observatory.",
"style": "The personal liability of the staff towards the Observatory shall be governed by the provisions applying to the staff of the Observatory.",
"zeroshot": "The personal liability of the employees towards the monitoring center is determined by the regulations applicable to the personnel of the monitoring center.",


some comet examples from high similarity to low:
{
    "src": "1. In Artikel 2 Absatz 1 wird der \"31. Mai 1996\" durch den \"31. Juli 1996\" ersetzt.",
    "tgt": "1. in Article 2, first subparagraph, '31 May 1996` is replaced by '31 July 1996`;",
    "bm": "1. In the first subparagraph of Article 2 (1), '31 May 1996` shall be replaced by '31 July 1996`.",
    "style": "In Article 2, paragraph 1, \"31 May 1996\" is replaced by \"31 July 1996\".",
    "zeroshot": "In Article 2 paragraph 1, \"May 31, 1996\" is replaced by \"July 31, 1996\".",
    "bm_bleu": 0.39160579612752916,
    "style_bleu": 0.2046592065585361,
    "zeroshot_bleu": 3.8992934777680458e-78,
    "bm_comet": 0.9141897559165955,
    "style_comet": 0.9042642712593079,
    "zeroshot_comet": 0.8741048574447632,
    "src_retrieve_de": "1. In Artikel 1 Absatz 3 Unterabsatz 2 wird der \"31. Dezember 1995\" durch den \"31. Dezember 1996\" ersetzt.",
    "src_retrieve_en": "1. In the second subparagraph of Article 1 (3), '31 December 1995` shall be replaced by '31 December 1996`.",
    "tgt_retrieve": "In Article 1, paragraph 3 is replaced by:",
    "comet": 0.9141897559165955
}

==> emnlp2023-latex/table_with_original_score.tex <==
\begin{table*}[]
\centering
\resizebox{0.8\linewidth}{!}{

\begin{tabular}{l|ccccccc|cc}
\hline
\multirow{2}{*}{Methods} & \multirow{2}{*}{bn} & \multirow{2}{*}{en} & \multirow{2}{*}{fi} & \multirow{2}{*}{id} & \multirow{2}{*}{ko} & \multirow{2}{*}{sw} & \multirow{2}{*}{avg.} & \multicolumn{2}{c}{\# params} \\ \cline{9-10} 
                         &                     &                     &                     &                     &                     &                     &                       & Training      & Inference     \\ \hline
Naive Multilingual       & 77.69               & 70.36               & 78.26               & 83.00               & 61.60               & 80.97               & 75.31                 & 270M          & 270M          \\
LMS, $d=32$              & 77.1                & 71.7                & 78.18               & 82.76               & 63.70               & 81.90               & 75.89                 & 279M          & 279M          \\
LMS+FD-LS, $d=32$    & 78.95               & \textbf{73.47}      & 78.80               & 84.27               & 61.90               & \textbf{81.35}      & 76.46                 & 280M          & 280M          \\
LMS+FD-Share, $d=32$   & \textbf{79.08}      & 73.44               & \textbf{78.86}      & \textbf{84.34}      & \textbf{62.15}      & 81.29               & \textbf{76.53}        & 280M          & 270M          \\ \hline
\end{tabular}
}
\caption{TODO: MQA results}
\label{tab:mqa_results}
\end{table*}


\begin{table}[]
\centering
\resizebox{1\linewidth}{!}{
% \begin{tabular}{lcccc}
% \hline
% \multirow{2}{*}{Methods} & \multirow{2}{*}{avg.} & \multirow{2}{*}{WR} & \multicolumn{2}{c}{\# params} \\
%                          &                       &                     & Training      & Inference     \\ \hline
% Naive Multilingual       & 89.20                 & -                   & 270M          & 270M          \\
% LMS, $d=32$              & 89.75                 & 96                  & 340M          & 340M          \\
% LMS+FD (Lang), d=32      & 89.87                 & 100                 & 343M          & 340M          \\
% LMS+FD (Share), d=32     & 89.53                 & 88                  & 343M          & 273M          \\ \hline
% \end{tabular}
\begin{tabular}{lcccccc}
\hline
\multirow{2}{*}{Methods} & \multicolumn{2}{c}{Sampled Language} & \multirow{2}{*}{avg.} & \multirow{2}{*}{WR} & \multicolumn{2}{c}{\# params} \\
                         & qu                & vi               &                       &                     & Tra.      & Inf.     \\ \hline
Naive MNER      & 76.79             & 92.60            & 89.20                 & -                   & 270M          & 270M          \\
LMS              & 80.40             & 92.88            & 89.75                 & 96                  & 340M          & 340M          \\
LMS+FD-LS      & 80.75             & 93.17            & 89.87                 & 100                 & 343M          & 340M          \\
LMS+FD-Share     & 80.01             & 93.05            & 89.53                 & 88                  & 343M          & 273M          \\ \hline
\end{tabular}
}
\caption{TODO: MNER results}
\label{tab:mner_results}
\end{table}

